Automated Analysis of MUTEX Algorithms with FASE

In this paper we study the liveness of several MUTEX solutions by representing them as processes in PAFAS s, a CCS-like process algebra with a specific operator for modelling non-blocking reading behaviours. Verification is carried out using the tool FASE, exploiting a correspondence between violations of the liveness property and a special kind of cycles (called catastrophic cycles) in some transition system. We also compare our approach with others in the literature. The aim of this paper is twofold: on the one hand, we want to demonstrate the applicability of FASE to some concrete, meaningful examples; on the other hand, we want to study the impact of introducing non-blocking behaviours in modelling concurrent systems.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{Giovanna D'Agostino, Salvatore La Torre (Eds.):\\
Proceedings of the Second International Symposium on\\ 
``Games, Automata, Logics and Formal Verification'' (GandALF 2011)\\
EPTCS 54, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.54.4}{10.4204/EPTCS.54.4}}
\pdfoutput=1

